A Column Generation based Heuristic for the Tail Assignment Problem

This article proposes an efficient heuristic in accelerating the column generation by parallel resolution of pricing problems for aircrafts in the tail assignment problem (TAP). The approach is able to achieve considerable improvement in resolution time for real life test instances from two major Indian air carriers. The different restrictions on individual aircraft for maintenance routing as per aviation regulatory bodies are considered in this paper. We also present a variable fixing heuristic to improve the integrality of the solution. The hybridization of constraint programming and column generation was substantial in accelerating the resolution process.

==> references.tex <==
@article{lapp2012incorporating,
  title={Incorporating aircraft efficiency measures into the tail assignment problem},
  author={Lapp, Marcial and Wikenhauser, Florian},
  journal={Journal of Air Transport Management},
  volume={19},
  pages={25--30},
  year={2012},
  publisher={Elsevier}
}

@article{maher2018daily,
  title={The daily tail assignment problem under operational uncertainty using look-ahead maintenance constraints},
  author={Maher, Stephen J and Desaulniers, Guy and Soumis, Fran{\c{c}}ois},
  journal={European Journal of Operational Research},
  volume={264},
  number={2},
  pages={534--547},
  year={2018},
  publisher={Elsevier}
}
@article{ruther2013integrated,
  title={Integrated aircraft routing, crew pairing, and tail assignment},
  author={Ruther, Sebastian},
  journal={Unpublished doctoral dissertation, University of Newcastle, Newcastle, Australia. http://nova. newcastle. edu. au/vital/access/manager/Repository/uon},
  volume={13585},
  year={2013}
}

@article{desaulniers1997daily,
  title={Daily aircraft routing and scheduling},
  author={Desaulniers, Guy and Desrosiers, Jacques and Dumas, Yvan and Solomon, Marius M and Soumis, Fran{\c{c}}ois},
  journal={Management Science},
  volume={43},
  number={6},
  pages={841--855},
  year={1997},
  publisher={INFORMS}
}
@article{du1999stabilized,
  title={Stabilized column generation},
  author={Du Merle, Olivier and Villeneuve, Daniel and Desrosiers, Jacques and Hansen, Pierre},
  journal={Discrete Mathematics},
  volume={194},
  number={1-3},
  pages={229--237},
  year={1999},
  publisher={Elsevier}
}
@article{gronkvist2006accelerating,
  title={Accelerating column generation for aircraft scheduling using constraint propagation},
  author={Gr{\"o}nkvist, Mattias},
  journal={Computers \& Operations Research},
  volume={33},
  number={10},
  pages={2918--2934},
  year={2006},
  publisher={Elsevier}
}
@article{desrochers1988generalized,
  title={A generalized permanent labelling algorithm for the shortest path problem with time windows},
  author={Desrochers, Martin and Soumis, Fran{\c{c}}ois},
  journal={INFOR: Information Systems and Operational Research},
  volume={26},
  number={3},
  pages={191--212},
  year={1988},
  publisher={Taylor \& Francis}
}
@article{marsten1975boxstep,
  title={The boxstep method for large-scale optimization},
  author={Marsten, Roy E and Hogan, WW and Blankenship, Jacob Watson},
  journal={Operations Research},
  volume={23},
  number={3},
  pages={389--405},
  year={1975},
  publisher={INFORMS}
}
@article{feo1989flight,
  title={Flight scheduling and maintenance base planning},
  author={Feo, Thomas A and Bard, Jonathan F},
  journal={Management Science},
  volume={35},
  number={12},
  pages={1415--1432},
  year={1989},
  publisher={INFORMS}
}
@article{borndorfer2010robust,
  title={Robust tail assignment},
  author={Bornd{\"o}rfer, Ralf and Dovica, Ivan and Nowak, Ivo and Schickinger, Thomas},
  year={2010}
}
@article{sarac2006branch,
  title={A branch-and-price approach for operational aircraft maintenance routing},
  author={Sarac, Abdulkadir and Batta, Rajan and Rump, Christopher M},
  journal={European Journal of Operational Research},
  volume={175},
  number={3},
  pages={1850--1869},
  year={2006},
  publisher={Elsevier}
}
@article{bacsdere2014operational,
  title={Operational aircraft maintenance routing problem with remaining time consideration},
  author={Ba{\c{s}}dere, Mehmet and Bilge, {\"U}mit},
  journal={European Journal of Operational Research},
  volume={235},
  number={1},
  pages={315--328},
  year={2014},
  publisher={Elsevier}
}
@book{gronkvist2005tail,
  title={The tail assignment problem},
  author={Gr{\"o}nkvist, Mattias},
  year={2005},
  publisher={Citeseer}
}
@article{liang2015robust,
  title={Robust weekly aircraft maintenance routing problem and the extension to the tail assignment problem},
  author={Liang, Zhe and Feng, Yuan and Zhang, Xiaoning and Wu, Tao and Chaovalitwongse, Wanpracha Art},
  journal={Transportation Research Part B: Methodological},
  volume={78},
  pages={238--259},
  year={2015},
  publisher={Elsevier}
}
@article{gabteni2009combining,
  title={Combining column generation and constraint programming to solve the tail assignment problem},
  author={Gabteni, Sami and Gr{\"o}nkvist, Mattias},
  journal={Annals of Operations Research},
  volume={171},
  number={1},
  pages={61},
  year={2009},
  publisher={Springer}
}

@article{gualandi2009constraint,
  title={Constraint programming-based column generation},
  author={Gualandi, Stefano and Malucelli, Federico},
  journal={4OR},
  volume={7},
  number={2},
  pages={113--137},
  year={2009},
  publisher={Springer}
}
@article{rousseau2004solving,
  title={Solving VRPTWs with constraint programming based column generation},
  author={Rousseau, Louis-Martin and Gendreau, Michel and Pesant, Gilles and Focacci, Filippo},
  journal={Annals of Operations Research},
  volume={130},
  number={1-4},
  pages={199--216},
  year={2004},
  publisher={Springer}
}
@article{gopalan1998mathematical,
  title={Mathematical models in airline schedule planning: A survey},
  author={Gopalan, Ram and Talluri, Kalyan T},
  journal={Annals of Operations Research},
  volume={76},
  pages={155--185},
  year={1998},
  publisher={Springer}
}

@article{barnhart2003applications,
  title={Applications of operations research in the air transport industry},
  author={Barnhart, Cynthia and Belobaba, Peter and Odoni, Amedeo R},
  journal={Transportation science},
  volume={37},
  number={4},
  pages={368--391},
  year={2003},
  publisher={INFORMS}
}
